LSTA-Net: Long short-term Spatio-Temporal Aggregation Network for Skeleton-based Action Recognition

Modelling various spatio-temporal dependencies is the key to recognising human actions in skeleton sequences. Most existing methods excessively relied on the design of traversal rules or graph topologies to draw the dependencies of the dynamic joints, which is inadequate to reflect the relationships of the distant yet important joints. Furthermore, due to the locally adopted operations, the important long-range temporal information is therefore not well explored in existing works. To address this issue, in this work we propose LSTA-Net: a novel Long short-term Spatio-Temporal Aggregation Network, which can effectively capture the long/short-range dependencies in a spatio-temporal manner. We devise our model into a pure factorised architecture which can alternately perform spatial feature aggregation and temporal feature aggregation. To improve the feature aggregation effect, a channel-wise attention mechanism is also designed and employed. Extensive experiments were conducted on three public benchmark datasets, and the results suggest that our approach can capture both long-and-short range dependencies in the space and time domain, yielding higher results than other state-of-the-art methods. Code available at https://github.com/tailin1009/LSTA-Net.

==> paperSec/abstract.tex <==
\begin{abstract}
% Modelling varied spatial-temporal dependencies is the key to recognising human actions in skeleton sequences. However, existing methods excessively rely on the design of traversal rules or graph topologies based on human prior knowledge to draw the dependency of dynamic joints, which is inadequate to reflect the important long-range spatial-temporal relationships due to the lack of contextual information between semantic parts and complex movement patterns in real skeletal data. To address the above problem, we propose a novel long short-term feature aggregation strategy to model long-range dependencies in spatial-temporal domain. Specifically, we devise our model into a factorised architecture which can alternately performs spatial feature aggregation and temporal feature aggregation. Furthermore, an additional attention module is proposed to enhance the aggregated features. As a result, our approach is capable of capturing both long and short range dependencies in space and time domain. Extensive experimental evaluation on three public benchmarks show that our method achieves comparable performance but keeps fewest parameters, demonstrating its efficiency in long-range dependency modeling.


Modelling varied spatial-temporal dependencies is the key to recognising human actions in skeleton sequences. However, existing methods excessively rely on the design of traversal rules or graph topologies based on human prior knowledge to draw the dependency of dynamic joints, which is inadequate to reflect the important long-range spatial-temporal relationships due to the lack of contextual information in real skeletal data. To address the above problem, we propose a novel long short-term feature aggregation strategy to model such long-range dependencies. Specifically, we devise our model into a factorised architecture which can alternately perform spatial feature aggregation and temporal feature aggregation. Furthermore, an additional attention module is proposed to enhance the aggregated features. As a result, our approach is capable of capturing both long-and-short range dependencies in the space and time domain. Extensive experimental evaluations on three public benchmarks show that our method achieves comparable performance but keeps fewest parameters, demonstrating its efficiency in long-range dependence modelling.


% Modelling varied spatial-temporal dependencies is the key to recognising human actions in skeleton sequences.
% However, the lack of contextual information between semantic parts and complex 

% Modelling varied spatial-temporal dependencies is the key to recognising human actions in skeleton sequences. However, existing methods excessively rely on the design of traversal rules or graph topologies based on human prior knowledge to draw the dependency of dynamic joints, which is inadequate to reflect the long-range spatial-temporal relationships in real skeletal data. 
% In this work, we present a novel  
% {\color{blue} long short-term aggregation network (LSTA-Net)} to effectively capture the sequence-independent long-range and {\color{blue} and short-term }correlations in skeletal data without the need of knowing the inherent positions of joints and the occurrence order of frames. 
% Our LSTA-Net consists of several LSTA {\color{blue}blocks}, each of which comprises of three main components, including spatial decentralized multi-scale aggregation module (SDA), temporal pyramid  aggregation module (TPA) and maximum-response attention module (MAM). SDA extracts the   disentangled structural features {\color{blue}in a decentralized manner}, and attaches MAM to capture long-range spatial semantics. 
% TPA deforms the local temporal convolution into a set of sub-convolutions, thus forming a pyramid residual architecture, which allows sub-convolutions to be successively applied to expand the equivalent receiving fields of temporal features and model their long-range temporal relationships over distant frames.
% MAM is almost a parameter-free attention module, which can effectively learn the features with the greatest response to the classifier and to be readily attached in both SDA and TPA modules to yield further improvements. To show the effectiveness of our method, we conducted extensive experiments and obtained better results than state-of-the-art methods on three challenging datasets, namely, NTU RGB+D, NTU RGB+D 120 and Kinetics-Skeleton 400.
\end{abstract}

==> paperSec/conclusion.tex <==
\section{Conclusion}
% 	In this paper, we propose to model both long-and-short-range spatial-temporal dependencies for skeleton-based action recognition with a novel long short-term aggregation  network (LSTA-Net). Our LSTA-Net involves three main components, including multi-scale spatial aggregation (MSA), temporal pyramid aggregation (TPA) and maximum-response attention module (MAM). The MSA module learns multiple disentangled spatial graphs. The TPA module can establish the reliable long-range temporal dependencies by deforming the local convolution into a set of sub-convolutions to enlarge the temporal receptive fields. MAM is an almost parameter-free local attention module, which can be easily integrated into both MSA and TPA to discover useful intrinsic spatial-temporal patterns. With extensive experiments on three skeletal datasets, we show that our model outperforms existing methods by sizable margins.   

We propose a factorised architecture which alternately performs spatial feature aggregation and temporal feature aggregation for efficient long short-term dependency modeling to skeleton-based action recognition. We develop three modules in our architecture: a multi-scale spatial aggregation (MSA), temporal pyramid aggregation (TPA) and maximum-response attention module (MAM). MAM is an almost parameter-free local attention module, which can be easily integrated into both MSA and TPA. Finally, we achieve comparable performances on three public benchmarks while keeping lowest model complexity.

==> paperSec/experiments.tex <==

	
\section{Experiments}
	
	\subsection{Datasets}
	

% 	2s-agcn 6.34
% ours 3.7
	
    % Following prior work \cite{shi2019two,msg3d}, 
    We evaluate our method on three public benchmark datasets: NTU RGB+D 60 \cite{ntu_60}, NTU RGB+D 120 \cite{ntu_120} and Kinetics-Skeleton \cite{kinetics}. 
    
    NTU RGB+D 60 and 120 contains 56,880 and 114,480 skeleton sequences corresponding to 60 and 120 action categories respectively. Each skeleton sequence contains the 3D spatial coordinate information of 25 joints captured by Microsoft Kinect v2 cameras. Cross-Subject(X-Sub) and Cross-View (X-View) in NTU RGB+D 60 and Cross-Subject(X-Sub) and Cross-Set (X-Set) in NTU RGB+D 120 are different evaluation settings for train-test split.
    
    Kinetics-Skeleton is a large-scale dataset sourced from the Kinetics 400 video dataset \cite{kinetics} by using the OpenPose\cite{cao2018openpose} pose estimation toolbox. Effective skeleton sequences are divided into two groups, 240,436 for training and 19,796 for testing. Each skeleton sequence contains the 2D spatial coordinate information of 18 joints and the corresponding confidence score. Details can be found in \cite{ntu_120,kinetics}
      
      
      
  
    
   
    % 主要介绍数据集什么场景采集，训练/测试样本多少，突出亮点
    
    
    
    % The algorithms are recommended to be evaluated under two benchmarked schemes, including Cross-subject (X-Sub) and Cross-view (X-View). For X-Sub settings, the data of a total of 40 subjects are split into training and testing groups, generating 40,091 and 16,487 training and testing samples, respectively. For X-View settings, 37,920 video clips captured from cameras 2 and 3 are used for training, while 18,960 video clips captured from cameras 1 are used for testing.   
    
% 	\noindent\textbf{NTU RGB+D} NTU RGB+D \cite{ntu_60} is one of the most frequently used in-door-captured action recognition dataset, which contains 56,880 skeleton sequences spanning 60 action categories. The fragments are collected from 40 individuals aged 10 to 35 years. Each bone sequence is represented by 25 joints, and the spatial information of these joints is captured by three Microsoft Kinect v2 cameras from different angles concurrently. The algorithms are recommended to be evaluated under two benchmarked schemes, including Cross-subject (X-Sub) and Cross-view (X-View). For X-Sub settings, the data of a total of 40 subjects are split into training and testing groups, generating 40,091 and 16,487 training and testing samples, respectively. For X-View settings, 37,920 video clips captured from cameras 2 and 3 are used for training, while 18,960 video clips captured from cameras 1 are used for testing.   

% 	\noindent\textbf{NTU RGB+D 120} NTU RGB+D 120 \cite{ntu_120} introduced an additional 57,367 skeleton sequences on the basis of NTU RGB+D dataset, making it dominant in the publicly available 3D joint annotation datasets. The dataset contains 114,480 skeleton samples covering 120 action categories. These samples are captured from 106 different subjects and 32 different camera setups. The setting of Cross-Subject is similar to the NTU RGB+D \cite{ntu_60}, which is to select half of the samples of the subjects for training ({i.e.,} 63,026), and then test the remaining samples ({i.e.,} 50,919). The settings of X-View are substituted by Cross-Setup (X-Set), in which 54, 468 samples collected from half of the camera setups are used for training and the remaining 59, 477 samples are used for testing.   
	
% 	\noindent\textbf{Kinetics-Skeleton} Kinetics-Skeleton \cite{st_gcn} is a large-scale dataset sourced from the Kinetics 400 video dataset \cite{kinetics} by using the OpenPose pose estimation toolbox. Effective skeleton sequences are divided into two groups, namely 240,436 for training and 19,796 for testing. Each skeleton sequence contains the 2D spatial coordinate information of 18 joints and the corresponding confidence score predicted by OpenPose \cite{cao2018openpose}. At each time step, the upper limit of the number of skeletons is 2, and skeletons with lower overall confidence are discarded. 
	\subsection{Implementation Details}
	The proposed LSTA-Net is implemented by PyTorch toolkit and run on a server with four TitanV GPU. The batch size is set to 64 (16 per worker). The model is trained for 100 epochs with Nesterov momentum (0.9) SGD and the cross-entropy loss. The initial learning rate is set to 0.05 and decayed with a factor of 0.1 at epochs \{40,60,80,100\}. The weight decay is set to 0.0005 for all experiments. The architecture is the same as the factorised path in \cite{msg3d} but with the different output channels (i.e., 72, 144 and 288 for each LSTA block in sequential). The kernels of adaptive maxpooling layer in MAM module are empirically set to 3 and 5 for A-SDA and A-TPA, respectively. The input skeletal data is padded to \textit{T}=300 frames by replaying the actions. All sequences are pre-processed with normalisation and translation that employed in \cite{shi2019skeleton,shi2019two,msg3d}. It is worth noting that none of the data augmentation methods is employed in our method. 
	
		\subsection{Comparison with State-of-the-arts}
% 	\begin{table}[]
% 		\centering
% 		\scalebox{0.84}{
% 			\begin{tabular}{lccc}
% 				\toprule
% 				\multirow{2}{*}{Methods} & \multirow{2}{*}{Publiser} &\multicolumn{2}{c}{NTU RGB+D 120} \\ \cline{3-4}
% 				& & X-Sub     & X-Set     \\  \midrule\midrule   
% 				PA-LSTM \cite{ntu_60}               &CVPR& 25.5           & 26.3            \\     
% 				ST-LSTM \cite{liu2016spatio}     &ECCV& 55.7           & 57.9            \\
% 				Clips+CNN+MTLN \cite{ke2017new}			&CVPR&58.4	&57.9\\
% 				2s-GCA-LSTM \cite{liu2017global}                &CVPR& 61.2           &63.3             \\
% 				2s-AGCN \cite{shi2019two}                 &CVPR& 82.9           & 84.9            \\
% 				RotClips+MTCNN \cite{ke2018learning}		&TIP&58.4&57.9\\
% 				\begin{tabular}[l]{@{}l@{}}Body Pose Evolution Map\\ \cite{liu2018recognizing}\end{tabular} &CVPR&64.6&66.9\\
% 				SGN \cite{zhang2020semantics}						 &CVPR& 79.2		   & 81.5			 \\
% 				2s-Shift-GCN \cite{cheng2020skeleton}             &CVPR& 85.3           & 86.6            \\
% 				\midrule
% 				\textbf{LSTA-Net (Joint+Bone)}         &-         & \textbf{86.70}           & \textbf{87.9}    		\\
% 				\bottomrule       
% 		\end{tabular}}
% 		\caption{\label{ntu120} Comparison of the Top-1 accuracy (\%) with the state-of-the-art methods on the NTU RGB+D 120 dataset. X-Sub and X-Setup denote the settings of cross-subject and cross-setup, respectively.}
% 	\end{table}
	
	\begin{table}[t!]
		\centering
		\scalebox{0.84}{
			\begin{tabular}{lcccc}
				\toprule
				\multirow{2}{*}{Methods} & \multirow{2}{*}{Publiser} &\multicolumn{2}{c}{Kinetics Skeleton} \\ \cline{3-4}
				& & Top-1     & Top-5     \\  \midrule\midrule   
				PA-LSTM \cite{ntu_60}               &CVPR& 16.4           & 35.3            \\ 
				TCN \cite{kim2017interpretable}			&CVPRW&20.3	&40.0\\
				ST-GCN \cite{st_gcn}                  &AAAI& 30.7           & 52.8            \\
				% STGR-GCN \cite{li2019spatio}                &AAAI& 33.6           & 56.1            \\
				AS-GCN \cite{li2019actional}                  &CVPR& 34.8           & 56.5            \\
				2s-AGCN \cite{shi2019two}                 &CVPR& 36.1           & 58.7            \\
				DGNN \cite{shi2019skeleton}                  &CVPR& 36.9           & 59.6            \\
				NAS-GCN \cite{peng2020learning}             	 &AAAI& 37.1           & 60.1            \\
				MS-G3D \cite{msg3d}                     &CVPR  &    38.0 & 60.9 \\     
				
				\midrule
				\textbf{LSTA-Net (Ours)}         &-         &  37.9           & 60.7   		\\
				\bottomrule
		\end{tabular}}
		\caption{Comparison of the Top-1 accuracy (\%) and Top-5 accuracy (\%) with the state-of-the-art methods on the Kinetics Skeleton dataset.}
		\vspace{-0.2cm}
		\label{kinetics}
	\end{table}

	We compare our full model with other state-of-the-art methods on NTU-RGB+D 60 \& 120 and Kinetics-Skeleton datasets in Tabel \ref{ntu60,120}. 
	{
	%\color{blue} In Tabel \ref{ntu60,120}, the Top-1 Accuracy of non-gcn methods and gcn-based methods are compared together. 
    As shown in Table \ref{ntu60,120}, our method outperforms conventional CNN and RNN based methods by a large margin.
    Our method also surpasses most GCN based methods, such as SGN \cite{zhang2020semantics}, NAS-GCN \cite{peng2020learning} and 2s-Shift-GCN \cite{cheng2020skeleton} and achieves comparable performance with MS-G3D \cite{msg3d}, which performs long-range aggregation with a multi-scale technique in unified spatial-temporal domain. However, our method utilizes factorised architecture and hence it is more light-weight. We additionally compare the number of model parameters  with several SOTA GCN models in Table \ref{ntu60,120}. The result shows that our proposed LSTA-Net has fewest parameters while keeping the SOTA performance, validating the effectiveness of our proposed factorised long short-term aggregation scheme.
    
    We show the experimental results of Kinetics-skeleton dataset in Table \ref{kinetics}. Our proposed LSTA-Net achieves comparable performance with MS-G3D and outperforms the others. As Kinetics-skeleton dataset has 240,436 training samples, given the fact that our model has only 1/3 parameters as in MS-G3D, the proposed long short-term aggregation strategy is validated to be efficient in such a large dataset.
    }
    
	 
% 	In particular, our method surpasses several GCN-based methods recently published at the top conference, including SGN \cite{zhang2020semantics}, NAS-GCN \cite{peng2020learning} and 2s-Shift-GCN \cite{cheng2020skeleton}. In addition, our method is largely superior to CNN-based methods and RNN-based methods (e.g., with about 10\% higher than Ind-RNN \cite{li2018independently} and Synthesized CNN \cite{liu2017enhanced} in the cross-subject setting). For the recently released large-scale dataset, i.e., NTU-RGB+D 120, our method once again obtains the best performance compared to the existing works listed (shown in Table \ref{ntu120}). Especially, our LSTA-Net surpasses the latest SGN \cite{zhang2020semantics} approach by 7.0\% and 6.4\% in the settings of cross-subject and cross-setup, respectively. From Table \ref{kinetics}, it is not difficult to find that our method remains in the leading position in terms of accuracy. Although NAS-GCN \cite{peng2020learning} presents strong competitiveness, it is still slightly lower than the proposed LSTA-Net.
	
% 	\begin{table}[]
% 	    \centering
% 	    \scalebox{0.85}{
% 		\begin{tabular}{lcccc}
% 			\toprule
% 			\multirow{2}{*}{Methods} & \multicolumn{4}{c}{Number of Scales} \\ \cline{2-5} & K=1     & K=4     & K=8     & K=12                                                                                \\ \midrule\midrule
% 			GCN         & 85.1    & 85.6    & 86.5      & 86.6  \\
% 			MS-GCN      & 85.1    & 87.0    & 86.9      & 86.8  \\ 
% 			Ours (SDA)  & 86.9     &87.8     & 88.3       & 88.1   \\
% 			\midrule
% % 			GCN-D       &85.1        &87.0         &86.9         &88.3  \\                                      
% % 			GCN-D+Mask &  86.1 & 86.9 & 87.9 & 87.8           
% % 			\\ 
% 			GCN+Mask        & 86.1  & 87.0    & 87.5    & 87.7 \\ 
% 			MS-GCN + Mask   & 86.1  & 86.9    & 87.9    & 87.8\\
% 			Ours (SDA+Mask) & 87.5  & 88.2    & 89.1    & 88.6          \\
% 			\bottomrule         
% 		\end{tabular}}
% 		\caption{Comparison of the Top-1 accuracy (\%) using different multi-scale aggregation methods in LSTA blocks with different $K$. "Mask" refers to the residual masks $ \widehat{\textbf{A}_{(k)}^{\rm{res}}} $ introduced in Eq.(\ref{eq12}). The performance is reported on NTU-RGB+D cross-sub setting using only the joint data.}
% 		\label{scales_and_para}
% 	\end{table}
	
	    
	\begin{table}[!t]
	    \centering
	    \scalebox{0.84}{
		\begin{tabular}{lcccc}
			\toprule
			\multirow{2}{*}{Spatial Aggregation Scheme} & \multicolumn{4}{c}{Number of Scales} \\ \cline{2-5} & K=1     & K=4     & K=8     & K=12                                                                                \\ \midrule\midrule
		    GCN       & 87.1  & 88.2    & 88.6    & 88.1  \\ 
		    MS-GCN\cite{msg3d}   & 87.1  & 88.2     & 89.0    & 88.2  \\
		    SDA (Ours) & 87.1  & 88.3   & \textbf{89.1}    & 88.2  \\
			\bottomrule         
		\end{tabular}}

		\vspace{-0.2cm}
	\end{table}
	

% 	\begin{table}[]
% 	    \centering
% 	    \scalebox{0.85}{
% 		\begin{tabular}{lcc}
% 			\toprule
% 			 Spatial Aggregation Scheme & Joint     & Bone \\ 
% 			\midrule \midrule
% %             Spatial Aggregation Scheme\\
% %                 % \quad with GCN        & --    & --    & --     & --  \\
% % 			    \quad with MS-GCN      & 95.1    & 95.3    & 88.6*     & 89.3  \\ 
% % 			    \quad with SDA (Ours) & 95.2     & 95.3     & 88.9*     & 89.5*   \\
% % 			\midrule 
% 			\\
% 			\quad with MS-TCN      & 88.7   & --  \\ 
% 			\quad with Ours (TPA)      & 89.1*     & 89.5*   \\
			
% 			\bottomrule         
% 		\end{tabular}}
% 		\caption{Comparison of the Top-1 accuracy (\%) with MS-TCN/MS-GCN}
% 		\label{compare_with_ms_tcn}
% 	\end{table}
	
	
	
	\begin{table}[t!]
	    \centering
	    \scalebox{0.85}{
		\begin{tabular}{lcc}
			\toprule
			Temporal Aggregation Scheme & Joint  \\
			\midrule \midrule
%             Spatial Aggregation Scheme\\
%                 % \quad with GCN        & --    & --    & --     & --  \\
% 			    \quad with MS-GCN      & 95.1    & 95.3    & 88.6*     & 89.3  \\ 
% 			    \quad with SDA (Ours) & 95.2     & 95.3     & 88.9*     & 89.5*   \\
% 			\midrule 
			MS-TCN\cite{msg3d}     & 88.7    \\ 
			TPA(Ours)      & \textbf{89.1}      \\
			\bottomrule
		\end{tabular}}
		\caption{Ablation study on temporal aggregation scheme. Numbers are Top-1 accuracy (\%).}
		\label{compare_with_ms_tcn}
		\vspace{-0.2cm}
	\end{table}
	

	
	\begin{table}[t!]
	    \centering
	    \scalebox{0.85}{
		\begin{tabular}{lccc}
			\toprule
			Methods              & Joint & Bone & Combine \\
			\midrule\midrule
			LSTA-Net (SDA \& TPA)     &94.2            &94.4           &95.3              \\
			LSTA-Net (A-SDA \& TPA)   &94.5            &94.8           &95.9              \\
			LSTA-Net (SDA \& A-TPA)   &95.0            &94.9           &96.0             \\
			LSTA-Net (A-SDA \& A-TPA) &\textbf{95.1}            &\textbf{95.3}           & \textbf{96.3}             \\
			\bottomrule
		\end{tabular}}
	\caption{Ablation study on maximum-response attention module(MAM). 'SDA' and 'TPA' represents raw spatial decentralized aggregation module and temporal pyramid aggregation module, without attention. 'A-SDA' indicates the 'SDA' added with our MAM, 'A-TPA' indicates 'TPA' added with our MAM. Results are the Top-1 accuracy (\%) under NTU RGB+D Cross-View setting.}
	\vspace{-0.2cm}
	\label{module_ablation_study}
	\end{table}
	
	
% 	\begin{table}[]
% 	    \centering
% 	    \scalebox{0.85}{
% 		\begin{tabular}{lccc}
% 			\toprule
% 			Methods              & Joint & Bone & Combine \\\midrule\midrule
% 			2s-AGCN \cite{shi2019two}              & 93.7       & 93.2      & 95.1         \\
% % 			NAS-GCN \cite{peng2020learning}              & 94.6       & 94.7      & 95.7         \\
% 	        MS-G3D \cite{msg3d}              & 95.0       & 95.3      & 96.2   \\ 			
% 			\midrule
% 			\textbf{LSTA (SDA \& TPA)}     &94.2            &94.4           &95.3              \\
% 			\textbf{LSTA (A-SDA \& TPA)}   &94.5            &94.8           &95.9              \\
% 			\textbf{LSTA (SDA \& A-TPA)}   &95.0            &94.9           &96.0             \\
% 			\textbf{LSTA (A-SDA \& A-TPA)} &\textbf{95.1}            &\textbf{95.3}           & \textbf{96.3}             \\
% 			\bottomrule
% 		\end{tabular}}
% 	\caption{ Comparison of the Top-1 accuracy (\%) on NTU RGB+D cross-view setting.}
% 	\label{module_ablation_study}
% 	\end{table}
	
	
	
	
	% Please add the following required packages to your document preamble:
	% \usepackage{multirow}
	\begin{table}[t!]
		\scalebox{0.96}{
		\begin{tabular}{lc|cccc|c|c}
			\toprule
			\multirow{3}{*}{MAM} & \multicolumn{7}{c}{Number of Dilation Rates}                        \\\cline{2-8}
			& K=3      & \multicolumn{4}{c}{K=5}            & K=7      & K=9      \\	\cline{2-8}
			& 1$\sim$3 & 1 & 1$\sim$2 & 1$\sim$3 & 1$\sim$4 & 1$\sim$3 & 1$\sim$3 \\
			\midrule\midrule 
			Acc                     &88.5          &87.4   &88.6          &\textbf{89.1}          &87.9          &88.4          &87.7        \\
			\bottomrule 
		\end{tabular}}
	\caption{Parameter selection of MAM. K denotes the kernel size of 1\textit{D} convolution, and 1$\sim$3 indicates the dilation rates of 1, 2 and 3.}
	\vspace{-0.2cm}
% 	\caption{Comparison of MAM accuracy (\%) using different dilation rates on the NTU RGB+D cross-subject setting. K denotes the kernel size of 1\textit{D} convolution, and 1$\sim$3 indicates the dilation rates of 1, 2 and 3.}
	\label{mam_ablation_study}
	\end{table}


\subsection{Ablation Study}
In this section, we report the results of our ablation study to validate the effectiveness of our proposed model components or strategies. 
Unless stated, performance is reported as classification accuracy on the Cross-Subject setting of NTU RGB+D 60 using only the joint data.

\noindent\textbf{Spatial Decentralized Aggregation (SDA)}
In Table \ref{compare_with_basic_ms_gcn}, we compare the proposed SDA with the basic adjacency powering method and disentangling \cite{msg3d} method in terms of the number of scales. We replace the spatial aggregation strategy of the LSTA blocks, referred to as "GCN", "MS-GCN" and "SDA", respectively. We observe that our decentralized aggregation strategy can outperform basic adjacency powering  method on different scales. 

\noindent\textbf{Temporal Pyramid Aggregation (TPA)}
%To explore the effectiveness of our LSTA-Net, we perform the ablation experiments on NTU RGB-D dataset. 
We also conduct ablation experiments on temporal aggregation schemes, and show the results in Table \ref{compare_with_ms_tcn}. From the table we can see that our proposed temporal pyramid aggregation scheme outperforms the direct aggregation as in MS-TCN\cite{msg3d}.

\noindent\textbf{Maximum-response Attention Module (MAM)}
We finally perform ablation studies on our proposed attention strategy. As shown in Table \ref{module_ablation_study}, our proposed MAM both improves SDA and TPA. We observe that adding MAM to TPA brings higher benefits than adding it to SDA, but simultaneously coupling the attention module helps to further improve accuracy. We additionally perform experiments on the parameter selection of MAM in our final LSTA-Net. As in Table \ref{mam_ablation_study}, we change kernel sizes and dilation rates of convolutions. With the guidance of experimental results, we finally set the 1\textit{D} convolution kernel size to 5 and dilate it three times at the rate of 1, 2 and 3.


% \subsubsection{Decentralized Multi-Scale Aggregation Method}
% In Table \ref{scales_and_para}, we compare the proposed spatial decentralized aggregation method (SDA)  in terms of the number of scales and model parameters. Using disentangled graph sources and the similar network architecture, our method can significantly outperform MS-G3D on different scales with fewer parameters. We also evaluated the effectiveness of attaching attention modules to different spatial and temporal aggregation modules in Table \ref{module_ablation_study} (i.e., A-MSA and A-TPA). Concretely, attaching the attention module to the TPA module brings higher benefits than adding it to the MSA module, but simultaneously coupling the attention module helps to further improve accuracy. In addition, the effectiveness of choosing different convolution kernel sizes and expansion ratios is illustrated in Table \ref{mam_ablation_study}. The best classification accuracy can be achieved by setting the kernel size of the 1\textit {D} convolution to 5 and dilating it three times at the rate of 1, 2 and 3. Either changing the kernel size or the number of dilation rates, the performance will be slightly reduced.    


{\color{black}
% In Table \ref{scales_and_para}, we compare the proposed spatial decentralized aggregation method with the basic multi-scale aggregation method in terms of the number of scales. We do so by replacing the spatial aggregation method of the LSTA blocks, referred to as "GCN" and "SDA", respectively. We observe that our method can significantly outperform basic adjacency powering  method on different scales. 

% We also evaluated the effectiveness of attaching attention modules to different spatial and temporal aggregation modules in Table \ref{module_ablation_study} (i.e., A-SDA and A-TPA). Concretely, attaching the attention module to the TPA module brings higher benefits than adding it to the SDA module, but simultaneously coupling the attention module helps to further improve accuracy. 

% In addition, the effectiveness of choosing different convolution kernel sizes and expansion ratios is illustrated in Table \ref{mam_ablation_study}. The best classification accuracy can be achieved by setting the kernel size of the 1\textit {D} convolution to 5 and dilating it three times at the rate of 1, 2 and 3. Either changing the kernel size or the number of dilation rates, the performance will be slightly reduced.
}


==> paperSec/intro.tex <==

	
\section{Introduction}
% 	Human action recognition, as one of the fundamental task in computer vision community, becomes increasingly demanding in a wide range of practical applications, such as video surveillance, behaviour analysis, video retrieval and human-computer interaction \cite{poppe2010survey,weinland2011survey}. With the advent of cost-effective depth cameras \cite{zhang2012microsoft} and advances in human pose estimation \cite{shotton2011real,cao2018openpose}, the cost of obtaining key points of the human body has been dramatically reduced, which has led to the increasing appeal of skeleton-based human motion recognition \cite{aggarwal2014human,st_gcn}. In particular, the representation of the skeleton is relatively low-dimensional but effective, and has the advantages of high abstraction and environmental robustness \cite{zhang2020semantics,zhang2020context,st_gcn}.

% action recognition is important ...
% in some scenarios, strongly correlated with skeleton, as 


%Human action recognition is a fundamental task in computer vision community, and it has a wide range of practical applications, such as behaviour analysis, video retrieval and human computer interaction\cite{poppe2010survey,weinland2011survey}. 




In recent years, skeleton-based action recognition has shown increasing interest to research community\cite{aggarwal2014human,st_gcn} due to the advent of cost-effective depth cameras \cite{zhang2012microsoft} and efficient human pose estimation methods\cite{cao2018openpose}. Compared with conventional RGB video based action recognition, the data structure of skeleton representation is in low-dimension and hence it can be easily stored in devices and transferred. In addition, skeletons also preserve people's privacy compared with RGB videos and can used in privacy sensitive scenarios, such as hospital or household surveillance cameras.

% 	Recently, substantial efforts have been devoted to extracting features from skeletal data by manually modelling the input skeleton sequence as a point-sequence based on joint coordinates \cite{du2015hierarchical,li2018independently,liu2016spatio,song2017end,zhang2017view}, or treating it as a pseudo image \cite{ke2017new,kim2017interpretable,liu2017enhanced}. The obtained features are subsequently fed into RNNs or CNNs for classification. However, bluntly treating skeletons as vector sequences or 2D grids cannot fully express the dependence between related joints. Considering the fact that the representation of human skeleton lies in a non-Euclidean space, a more natural method is to model the relationship between joints through a graph neural networks (GNNs). In view of the vigorous development of convolution operations, graph convolutional networks (GCN) are gradually introduced to solve the problem of skeleton-based action recognition. In particular, \cite{st_gcn} proposed a breakthrough work named ST-GCN, which constructed a spatial graph based on the natural connections of human joints and introduced temporal edges between corresponding joints in consecutive frames. Many of the latest works \cite{li2019spatio,li2019actional,shi2019skeleton,shi2019two,si2019attention,wen2019graph,msg3d} can be regarded as variants of ST-GCN, where they typically applied different functional modules to enhance feature expression and classification performance.


	\begin{figure}[!tbp]
		\centering
		\includegraphics[width=0.4\textwidth]{figures/ads.pdf}
		\caption{Architecture comparison between MS-G3D(left)\cite{msg3d} and proposed LSTA-Net(right). MS-G3D captures spatial and temporal dependencies in a unified G3D module, but it still requires the factorized pathway to be alongside, hence consists of multiple pathways. Our LSTA-Net utilizes the attention module (MAM) to enhance spatial aggregation and temporal aggregation. It is more lightweight since it only has single pathway.}
		\vspace{-0.3cm}
		\label{fig:ad}
	\end{figure}

Skeleton-based action recognition is a challenging task due to the lack of context information compared with RGB video based action recognition. In particular, modeling long range dependencies in spatial and temporal dimensions are difficult due to the flexible configuration between different semantic parts, as well as complex movement patterns in time domain.
Early works adopt sequential models to model joint relations, which first extract features of frames by treating joints as pixels and then utilize RNN-based models to model temporal relationships\cite{du2015hierarchical,liu2016spatio}. Another bunch of works concatenate skeletons of different time steps to generate a pseudo image, and utilize CNNs to perform image-based classification\cite{ke2017new,kim2017interpretable}. However, human skeletons are not in an Euclidean space and hence above methods cannot model joint dependencies efficiently. A more natural method is to model the relationship between joints through a graph neural networks (GNNs). In view of the vigorous development of convolution operations, graph convolutional networks (GCNs) are gradually introduced to solve the problem of skeleton-based action recognition. In particular, \cite{st_gcn} proposed a breakthrough work named ST-GCN, which constructed a spatial graph based on the natural connections of human joints and introduced temporal edges between corresponding joints in consecutive frames. Many of the latest works \cite{li2019spatio,li2019actional,shi2019two,si2019attention,wen2019graph} can be regarded as variants of ST-GCN, where they typically applied different functional modules to enhance feature expression and classification performance.

% 	Recently, substantial efforts have been devoted to extracting features from skeletal data by manually modelling the input skeleton sequence as a point-sequence based on joint coordinates \cite{du2015hierarchical,li2018independently,liu2016spatio,song2017end,zhang2017view}, or treating it as a pseudo image \cite{ke2017new,kim2017interpretable,liu2017enhanced}. The obtained features are subsequently fed into RNNs or CNNs for classification. However, bluntly treating skeletons as vector sequences or 2D grids cannot fully express the dependence between related joints. Considering the fact that the representation of human skeleton lies in a non-Euclidean space, a more natural method is to model the relationship between joints through a graph neural networks (GNNs). In view of the vigorous development of convolution operations, graph convolutional networks (GCN) are gradually introduced to solve the problem of skeleton-based action recognition. In particular, \cite{st_gcn} proposed a breakthrough work named ST-GCN, which constructed a spatial graph based on the natural connections of human joints and introduced temporal edges between corresponding joints in consecutive frames. Many of the latest works \cite{li2019spatio,li2019actional,shi2019skeleton,shi2019two,si2019attention,wen2019graph,msg3d} can be regarded as variants of ST-GCN, where they typically applied different functional modules to enhance feature expression and classification performance.

Despite the significant improvements in performance, there exist some limitations in the above methods. Specifically, both recurrent and convolutional operations are based on local neighbours in the space or time domain. The capture of long-range dependencies only can be achieved by repeatedly performing these operations and gradually propagating signals through the data and hence is inefficient. Recent work MS-G3D \cite{msg3d} proposed a unified spatial-temporal operator to model the long term dependencies in space and time domain. However, the proposed G3D module relies on its original factorised pathway and the overall operator has multiple pathways and hence leads to complex model architecture.

In this paper, we propose a novel long short-term feature aggregation strategy to model long-range dependencies between spatial and temporal domain. Different from the unified operation as in MS-G3D, we adopt a purely factorised framework which first aggregates features in spatial dimension and then performs temporal aggregation. To model the long range dependencies in spatial domain, we propose a novel multi-scale aggregation scheme; as in temporal long range modeling, we enlarge the receptive fields in temporal dimension by combing temporal convolution with different dilation rates, and additionally a novel temporal pyramid structure is proposed for efficient feature aggregation. We further propose a novel attention mechanism to enhance the spatial and temporal features after the spatial aggregation and temporal aggregation. The spatial aggregation and temporal aggregation are alternately performed to achieve effective long range dependency modeling and finally the node features are pooled together to perform classification.


% For skeletal data, long-range correlations are crucially important but difficult to capture due to varied semantics (i.e., the type of joint and its relative position in the spatial-temporal domain). Intuitively, for the same two joints, different spatial coordinates usually convey very different semantics. For example, if the hand joint is above or in front of the head joint, the action is likely to be \textit{brushing hair} or \textit{brushing teeth}, respectively. Analogically, in the temporal dimension, the semantics are presented in a dynamic form and may differ only in the occurrence order of the frames, such as \textit{put on/take off jacket, a shoe or glasses} and \textit{sit down/stand up}. In order to capture long-range dynamic semantics, existing methods either construct inefficient hierarchical structures \cite{li2018co,hussein2013human,du2015hierarchical} or stack multiple convolution layers with intensive parameters \cite{msg3d}. However, the problem still remains if there exist back-and-forth semantic dependencies.

% Despite the significant improvements in performance, there exist some limitations in the above methods. Specifically, both recurrent and convolutional operations are based on local neighbours in the space or time domain. The capture of long-range dependencies only can be achieved by repeatedly performing these operations and gradually propagating signals through the data. For skeletal data, long-range correlations are crucially important but difficult to capture due to varied semantics (i.e., the type of joint and its relative position in the spatial-temporal domain). Intuitively, for the same two joints, different spatial coordinates usually convey very different semantics. For example, if the hand joint is above or in front of the head joint, the action is likely to be \textit{brushing hair} or \textit{brushing teeth}, respectively. Analogically, in the temporal dimension, the semantics are presented in a dynamic form and may differ only in the occurrence order of the frames, such as \textit{put on/take off jacket, a shoe or glasses} and \textit{sit down/stand up}. In order to capture long-range dynamic semantics, existing methods either construct inefficient hierarchical structures \cite{li2018co,hussein2013human,du2015hierarchical} or stack multiple convolution layers with intensive parameters \cite{msg3d}. However, the problem still remains if there exist back-and-forth semantic dependencies.

Specifically, in space domain, a decentralized multi-scale aggregation module(SDA) is used to do multi-scale disentangling, decentralized normalization and spatial aggregation of the neighbourhood on a given node. In temporal dimension, inspired by \cite{res2net}, we propose a temporal pyramid aggregation module(TPA) to model long-range temporal dynamics by deforming the ordinary convolution layer into a set of sub-convolutions and formulating them with a pyramid structure allowing residual connections between adjacent subsets. Our attention module, namely maximum-response attention module(MAM), improves the local cross-channel interaction via multiple high efficient 1-D convolutions as inspired by \cite{eca}. In our model architecture, SDA and three TPAs are stacked together to form a LSTA block, both SDA and TPA are enhanced with MAMs. Finally, we concatenate multiple LSTA blocks for better relation modeling. Our model is factorised in spatial and temporal domain. Its overall structure only has single pathway and hence it is light weight. We refer our overall model as long short-term aggregation network(\textit{LSTA-Net}). An illustration of our architecture and MS-G3D is shown in Figure \ref{fig:ad}. We evaluate our proposed method on three public benchmarks: NTU-RGB+D\cite{ntu_60}, NTU-RGB+D 120\cite{ntu_120} and Kinetics Skeletons\cite{kinetics}. The results show that our method achieves comparable performances but our model is more light weight than other methods.
The main contributions of our work lie in three folds:

\begin{itemize}

\item We propose a simple but efficient factorised GCN structure to capture long range dependencies between skeletal joints.
\item We instantiate our factorised structure by proposing a novel multi-scale spatial aggregation module (SDA), a temporal aggregation module (TPA), and an attention module (MMA) to enhance spatial and temporal features.
\item The experiments on three public benchmarks show that our proposed method achieves comparable performances but keeps fewest parameters, validating the efficiency of our method.
\end{itemize}  


%  Our LSTA-Net consists of three modules, including spatial decentralized multi-scale spatial aggregation module (SDA), temporal pyramid aggregation module (TPA) and maximum-response attention module (MAM) that can be applied to mutually enhance the capabilities of SDA and TPA modules. Specifically, SDA learns to aggregate multi-scale spatial information of disentangled neighbouring joints in a decentralized way. Inspired by \cite{res2net}, we propose TPA module to model long-range temporal dynamics by deforming the ordinary convolution layer into a set of sub-convolutions and formulating them with a pyramid structure allowing residual connections between adjacent subsets. Therefore, our TPA module can greatly expand the equivalent receptive fields of adjacent sub-convolutions and realise multiple information exchanges between adjacent frames without using stacked multi-layer convolutions. In addition, we also provide an attention module that based on \cite{eca}, which improves the local cross-channel interaction via multiple high efficient 1\textit{D} convolutions. The main contributions of our work lie in {\color{blue} five} folds:
	
	
% 	To address the aforementioned problems, we propose a long short-term aggregation network (LSTA-Net), which can explicitly capture the dynamic long-range {\color{red} as well as short-term} spatial-temporal dependencies without the requirement of knowing the intrinsic semantics of joints. Our LSTA-Net consists of three modules, including spatial decentralized multi-scale spatial aggregation module (SDA), temporal pyramid aggregation module (TPA) and maximum-response attention module (MAM) that can be applied to mutually enhance the capabilities of SDA and TPA modules. Specifically, SDA learns to aggregate multi-scale spatial information of disentangled neighbouring joints in a decentralized way. Inspired by \cite{res2net}, we propose TPA module to model long-range temporal dynamics by deforming the ordinary convolution layer into a set of sub-convolutions and formulating them with a pyramid structure allowing residual connections between adjacent subsets. Therefore, our TPA module can greatly expand the equivalent receptive fields of adjacent sub-convolutions and realise multiple information exchanges between adjacent frames without using stacked multi-layer convolutions. In addition, we also provide an attention module that based on \cite{eca}, which improves the local cross-channel interaction via multiple high efficient 1\textit{D} convolutions. The main contributions of our work lie in {\color{blue} five} folds:
	
% 	\begin{itemize}
	
% 	\item We propose a novel LSTA-Net to capture long-range spatial-temporal correlations in dynamic skeletal data by pyramidal aggregation of attentive graph features. 
% 	 {\color{blue}
% 	\item We design a novel spatial aggregation method which can capture the disentangling representations from   multiple scales.
%  	}
% 	\item We introduce the TPA module to effectively and efficiently enlarge the equivalent temporal receptive fields for long-range dependencies modelling. 
% 	\item We present a nearly parameter-free attention module MAM, which can be readily equipped in SDA and TPA modules to discover useful patterns with the greatest response to classification.
% 	\item The proposed LSTA-Net can achieve state-of-the-art performance on the experimental datasets with only needs to introduce a very limited number of parameters.
% 	\end{itemize}  



==> paperSec/method.tex <==
		
\section{Long Short-term Aggregation Network}
	\subsection{Multi-scale Decentralized Spatial Aggregation}
	A graph is defined as $\mathcal{G}=(\mathcal{V}, \mathcal{E})$, where $\mathcal{V}$ is the set of vertices and $\mathcal{E} \subseteq (\mathcal{V} \times \mathcal{V})$ is the set of edges. The relationship of the graph is represented by the graph adjacency matrix$\mathbf{A} \in \mathbb{R}^{N \times N}$ with a 1 or 0 in position $(v_{i}, v_{j})$according to whether $v_{i}$and $v_{j}$ are adjacent or not, where \textit{N} denotes the number of vertexes. $\mathbf{A}$ is a symmetric matrix while $\mathcal{G}$ is an undirected graph. Human graph sequences contain a set of node features $\mathcal{X}=\{{x}_{t}^{n}|1\leq n \leq N, 1\leq t \leq T; n, t \in \mathbb{Z}\}$ represented as a feature tensor $\textbf{X} \in \mathbb{R}^{N \times T \times C}$, where $x_{t}^{n}=\textbf{X}_{t}^{n}$ denotes the \textit{C} dimensional features of the node $ v_{n} $ at time \textit{t}. Let \textbf{W} $\in \mathbb{R}^{C_{\rm{in}} \times C_{\rm{out}}}$ be the learnable transformation matrix. Then, the spatial convolution on a given graph can be implemented similar to the convolution on a regular grid graph like an RGB image. Formally, the multi-scale GCN can be expressed as:  
	
	\begin{equation}\label{eq1}
	\textbf{X}_{t}^{\rm{spat}} = \sigma \left( \sum_{k=0}^{K} \widetilde{\textbf{A}_{k}} \textbf{X}_{t} \textbf{W}_{k} \right),
	\end{equation}
	where $ \textbf{X}_{t} \in \mathbb{R}^{N \times C_{\rm{in}}}$ and $ \textbf{X}_{t}^{\rm{spat}} \in \mathbb{R}^{N \times C_{\rm{out}}} $ denote the input and output skeleton features for \textit{t}-th frame, respectively. \textit{K} indicates the number of scales of the graph to be aggregated. $\sigma(\cdot)$ is the activation function. $\tilde{\textbf{A}}$ is the normalised adjacency matrix \cite{kipf2016semi,li2019actional} and can be obtained by: $\tilde{\textbf{A}}=\hat{\textbf{D}}^{-\frac{1}{2}}\hat{\textbf{A}}\hat{\textbf{D}}^{-\frac{1}{2}}$, where $\hat{\textbf{A}}=\textbf{A}+\textbf{I}$ is the adjacency matrix including the nodes of the self-loop graph and $\hat{\textbf{D}}$ is the degree matrix of \textbf{A}.   
% 		\begin{figure}[!tbp]
% 		\centering
% 		\includegraphics[width=0.45\textwidth]{FormattingGuidelines-IJCAI-21/figures/method_1.pdf}
% 		\caption{Visualization comparison of the \textbf{naive aggregation scheme} (Top), the \textbf{disentangling aggregation scheme} (Middle) \cite{msg3d} and the proposed \textbf{decentralized aggregation scheme} (Bottom). \textit{K} denotes the neighboring scale of a given node.}
% 		\label{fig:disentangled}
% 	\end{figure}
	The term of $ \widetilde{\textbf{A}_{k}} \textbf{X}_{t} $ in Eq.(\ref{eq1}) describes a weighted average feature that is based on the \textit{k}-order neighbourhood of the selected graph node. However, conventional multi-scale aggregation based on cyclic \textit{k}-hop neighbours will make low-order neighbours overweight and vice versa. %See Fig.\ref{fig:disentangled} for illustration. 
	Similar to \cite{msg3d}, we propose a novel decentralized multi-scale disentangling scheme to tackle with the bias weighting problem by introducing multiple scales rather than neighboring scales. Concretely, the elements of \textit{k}-adjacency matrix $ \widetilde{\textbf{A}_{(k)}} $ are first assigned the value 1 if $ v_{i} $ and $ v_{j} $ are adjacent or their shortest distance is equal to \textit{k} (i.e., $ d(v_{i}, v_{j}) =k$). Then, for those elements whose shortest distance lower/shorter than \textit{k} (i.e., $ d(v_{i}, v_{j}) < k$), are assigned with a scale-adaptive value $  \frac{d(v_{i}, v_{j})}{k}$. Finally, the rest of elements are set to 0. Thus, $ \widetilde{\textbf{A}_{(k)}} $ can be directly obtained by calculating the residuals of the matrix powers of current graph scale and the mean of previous graph scales:
	
% 	This bias weighting problem can be solved by disentangling the neighbourhood of a given node \cite{msg3d}. Concretely, the elements of \textit{k}-adjacency matrix $ \widetilde{\textbf{A}_{(k)}} $ are assigned the value 1 if $ v_{i} $ and $ v_{j} $ are adjacent or their shortest distance is equal to \textit{k} (i.e., $ d(v_{i}, v_{j}) =k$), and 0 otherwise. Thus, $ \widetilde{\textbf{A}_{(k)}} $ can be easily obtained by calculating the residuals of the matrix powers of neighbouring graph scales:
	
	
% 	\begin{equation}\label{eq2}
% 	\widetilde{\textbf{A}_{(k)}}=\textbf{I}+\mathbbm{1} \left(\widetilde{\textbf{A}_{k}}\geq 1\right)-\mathbbm{1} \left(\widetilde{\textbf{A}_{k-1}} \geq 1\right),
% 	\end{equation}
% 	where $\widetilde{\textbf{A}_{(1)}}=\widetilde{\textbf{A}}$ and $\widetilde{\textbf{A}_{(1)}}=\textbf{I}$. 
	
	
% 	However, in Eq.(\ref{eq2}), 
% 	$ \widetilde{\textbf{A}_{(k)}} $  only consider the \textit{difference} of neighbouring graph powers. We argue that such graph representation for different scales limit/hinder the robust expressions. Thus, we expand such representation from neighbouring graph scales to multiple scales.

	\begin{equation}\label{decentralized}
	\widetilde{\textbf{A}^*_{(k)}} = \textbf{I} + \mathbbm{1} \left(\widetilde{\textbf{A}_{k}}\geq 1\right) -\mathbbm{1} \left( ({ \frac{1}{k}} {\sum ^{k-1}_{n=0}}{\widetilde{\textbf{A}_{n}}})\geq 1 \right).
	\end{equation}	  
	where $\widetilde{\textbf{A}^{*}_{(1)}}=\widetilde{\textbf{A}}$ and $\widetilde{\textbf{A}^{*}_{(0)}}=\textbf{I}$. Then, the spatial decentralized multi-scale aggregation can be rewritten by substituting $\widetilde{\textbf{A}_{k}}$ with $\widetilde{\textbf{A}^{*}_{(k)}}$ in Eq. (\ref{eq1}):
	
	\begin{equation}\label{eq3}
		\textbf{X}_{t}^{\rm{spat}} = \sigma \left( \sum_{k=0}^{K} \widetilde{\textbf{A}^{*}_{(k)}} \textbf{X}_{t} \textbf{W}_{(k)} \right),
	\end{equation}  
	
		
	
    	\begin{figure*}[!htbp]
		\centering
		\includegraphics[width=0.9\textwidth]{FormattingGuidelines-IJCAI-21/figures/Framework_aa.pdf}
		\caption{An illustration of the proposed LSTA-Net, which consists of three LSTA blocks totally. Each LSTA block is comprised of one A-SDA module and three A-TPA modules. The kernel of adaptive max pooling layer is empirically set to 3 and 5 for A-SDA and A-TPA, respectively. DR means the different dilation rates. $\bigoplus$ and $\bigotimes$ denote element-wise addition and multiplication, respectively.}
		\label{fig:framework}
	    \end{figure*}
	      
	\subsection{Temporal Pyramid Aggregation}   
	Previously, most methods for recognising skeleton sequences adopted the local temporal convolution to process neighbouring frames at a time.  \cite{st_gcn,shi2019two,li2019spatio,li2019actional,shi2019skeleton}, 
	while the capture of long-range temporal information was rarely investigated or required a large number of stacked local operations to achieve\cite{msg3d}. 
% 	These methods cannot effectively or efficiently deal with the complex spatial-temporal relationships since the optimised message transmitted from distant frames can be dramatically weakened. 
	To capture the long-range dependencies in an efficient way and inspired by Res2Net \cite{res2net}, we propose the Temporal Pyramid Aggregation module (TPA) which can divide the convolution operation of the input features into a group of subsets. Consequently, the model effectively expand the equivalent receptive field of the temporal dimension without introducing additional parameters and time-consuming operations. 
	
	As shown in Figure \ref{fig:framework}, given the aggregated spatial graph feature $ \textbf{X}_{t}^{\rm{spat}} $, it  generates multiple fragments according to the local temporal convolution. The channel dimension of each fragment thus becomes \textit{C/s}, where \textit{s} is set to 6 empirically. Except for the first fragment, the remaining fragments are sequentially processed by temporal convolutions with gradually increasing dilation rates. Each fragment only has \textit{1/s} parameters as the original temporal convolution. The residual connections are applied to the neighbouring fragments to avoid the inconsistent information flow. Formally, this process can be written as: violate
	\begin{equation}\label{eq4}
	\begin{aligned}
	&\textbf{X}_{s}^{\rm{temp}}=\textbf{X}_{s}, \qquad \qquad \qquad \qquad \qquad \qquad \qquad s=1,\\
	&\textbf{X}_{s}^{\rm{temp}}=conv_{\rm{temp}}*\textbf{X}_{s}, \qquad \qquad \qquad \qquad \quad \ s=2,\\
	&\textbf{X}_{s}^{\rm{temp}}=conv_{\rm{temp}}*\left(\textbf{X}_{s}+\textbf{X}_{s-1}^{o}\right), \qquad s=3,4,5,6,
	\end{aligned}
	\end{equation}     
	where $ \textbf{X}_{s}^{\rm{temp}} $ is the output of \textit{s}-th fragment. $ conv_{\rm{temp}} $ denotes the 3$\times$1 temporal sub-convolution. For simplicity, we omit the subscript \textit{t} of $ \textbf{X}_{ts} $ in Eq.(\ref{eq4}).           
	
	The above operations endow the different fragments with different receptive fields in temporal dimension.The final output is easily obtained by concatenating outputs of multiple fragments and can be denoted as:
	\begin{equation}\label{eq5}
	\textbf{X}^{\rm{temp}}=[\textbf{X}_{1}^{\rm{temp}};\textbf{X}_{2}^{\rm{temp}};\textbf{X}_{3}^{\rm{temp}};\textbf{X}_{4}^{\rm{temp}};\textbf{X}_{5}^{\rm{temp}};\textbf{X}_{6}^{\rm{temp}}].
	\end{equation}
	
	The obtained feature $ \textbf{X}^{\rm{temp}} $ captures various ranges of spatial-temporal relationships, and are theoretically superior to a single local convolution in most existing approaches.  
	
	\subsection{Maximum-response Attention Module} 
	Human skeleton sequences comprise a limited number of dynamic key joints, which supplies a favourable breeding ground for the development of attention mechanisms. Specifically, a significant advantage of employing attention mechanism is that it can spontaneously and arbitrarily capture useful intrinsic correlations without knowing the content of the input sequence. Furthermore, since only the key joints are involved, the computational complexity of applying the attention mechanism is relatively small \cite{cho2020self}. These motivate us to explore an effective and efficient attention mechanism to extract the semantic dependence of skeletal data. Inspired by \cite{eca}, we propose a novel Maximum-response Attention Module that can be readily employed in standard CNNs-based architectures. Given an input feature  
	$ \textbf{X} \in \mathbb{R}^{ N \times T \times C} $, the channel attention can be computed as:
	\begin{equation}\label{eq6}
	\bm\omega=\tau \left( \textbf{W} g(\textbf{X})\right),
	\end{equation}
	where $\tau(\cdot)$ is the Sigmoid function and \textbf{W} is a $C \times C$ transformation matrix. $g(\textbf{X})$ denotes the function of channel-wise pooling. 
% 	For example, the Global Average Pooling (GAP) function can be denoted as: $g(\textbf{X})=\frac{1}{NT}\sum_{n=1,t=1}^{N,T}\textbf{X}_{nt}$. 
% 	As suggested by \cite{eca}, the local cross-channel interaction guarantees both efficiency and effectiveness, we thereby substitute \textbf{W} with a band $ \textbf{W}_{\eta} $ as follows:   
% 	\begin{equation}\label{eq7}
% 	\resizebox{.99\hsize}{!}{$ \left[\begin{array}{cccccccc}
% 	w^{1,1} & \ldots & w^{1, \eta} & 0 & 0 & \cdots & \cdots & 0 \\
% 	0 & w^{2,2} & \cdots & w^{2, \eta+1} & 0 & \cdots & \cdots & 0 \\
% 	\vdots & \vdots & \vdots & \vdots & \ddots & \vdots & \vdots & \vdots \\
% 	0 & \cdots & 0 & 0 & \cdots & w^{C, C-\eta+1} & \cdots & w^{C, C}
% 	\end{array}\right], $}
% 	\end{equation}
% 	where $ \eta $ is the kernel size and the size of parameter matrix $ \textbf{W}_{\eta} $ is $\eta \times C$. The weight matrix $ \textbf{W}_{\eta} $ only considers the interaction between $ y_ {i} $ and its $ \eta $ neighbours, and it could be more efficient to allow all channels to share learning weights. Concretely, we can write it as:
% 	\begin{equation}\label{eq8}
% 	\omega_{i}=\tau\left(\sum_{j=1}^{\eta} w^{j} y_{i}^{j}\right), y_{i}^{j} \in \Omega_{i}^{\eta},
% 	\end{equation}
% 	where $ \Omega_{i}^{\eta} $ is the set of $ \eta $ adjacent channels of $ y_{i} $.
Coincidentally, this can be implemented by the standard 1\textit{D} convolution with kernel size of $ \eta $. Then, we can rewrite Eq.(\ref{eq6}) in the form of:
	\begin{equation}\label{eq9}
		\bm\omega=\tau \left( conv1D_{\eta}\left(g(\textbf{X})\right)\right).
	\end{equation}
	
	The above operation only involves the $ \eta $ parameter, which is insignificant compared with the number of parameters of the entire network. However, the 1\textit{D} convolution equipped with a single convolution kernel can only provide a limited receptive field, which leads to insufficient local information interaction. To tackle this problem, we extend the 1\textit{D} convolution to a parallel fashion with different dilation rates. Subsequently, we apply the element-wise maximum operator to obtain the highest response of the input feature to the classifier. We propose to formulate this manipulation in the following manner:
	\begin{equation}\label{eq10}
	\bm\omega_{max}=\max_{\phi \in \Phi}\left(\phi(\bm\omega) \right),	
	\end{equation}
	where $\phi(\bm\omega)$ represents a set of 1\textit{D} convolutions stacking with different dilation rates, and $\Phi$ is the total length of attending convolutions. The new features $ \bm\omega_{max} $ is constructed in such a way not only enhances the interactivity of information, but also makes their output independent of the receptive fields known in advance by the various kernels.  
		\begin{table*}[ht!]
		\centering
		\scalebox{0.9}{
			\begin{tabular}{lc|c|cc|cc}
				\toprule
				\multirow{2}{*}{Methods} & \multirow{2}{*}{Publiser} & 
				% \multirow{2}{*}{FLOPs} 
				 \multirow{2}{*}{Param.} & \multicolumn{2}{c}{NTU RGB+D 60} & \multicolumn{2}{c}{NTU RGB+D 120} 
				\\ \cline{4-5} \cline{6-7}  & & & X-Sub & X-View & X-Sub & X-Set    
				\\  \midrule\midrule
				% \multicolumn{8}{c}{CNN and RNN based methods} \\
				% \\ \hline 
				% CNN and RNN based \\ 
				%  HBRNN \cite{du2015hierarchical}         &CVPR    &  &  59.1 & 64.0 & --    & --      \\
				PA-LSTM \cite{ntu_60}                   &CVPR    & -- &  60.7 & 67.3 & 25.5  & 26.3    \\
			    ST-LSTM \cite{liu2016spatio}            &ECCV    & -- &  69.2 & 77.7 & 55.0  & 57.9    \\
				% STA-LSTM \cite{song2017end}             &AAAI &  &  &  73.4 & 81.2 & --    & --      \\
				% GCA-LSTM \cite{liu2017global}           &CVPR &  &  &  74.4 & 82.8 & --    & --      \\
				 VA-LSTM \cite{zhang2017view}            &ICCV    & -- &  79.4 & 87.6 & --    & --      \\
				%  ARRN-LSTM \cite{zheng2019relational}    &ICME    &  &  80.7 & 88.8 & --    & --      \\
				% Ind-RNN \cite{li2018independently}      &CVPR &  &  &  81.8 & 88.0 & --    & --      \\
				TCN \cite{kim2017interpretable}         &CVPRW   & -- & 74.3 & 83.1 & --    & --      \\
				
				AGC-LSTM \cite{si2019attention}         &CVPR    & -- &  89.2 & 95.0 & --    & --      \\ 
				% Clips+CNN+MTLN \cite{ke2017new}         &CVPR &  &  &  79.6 & 84.8 & 58.4  & 57.9    \\
				\midrule\midru
                % \multicolumn{8}{c}{GCN based methods} 
				%  \midru
				 ST-GCN \cite{st_gcn}                    &AAAI   & 3.10 &  81.5 & 88.3 & 70.7  & 73.2    \\
				% STGR-GCN \cite{li2019spatio}            &AAAI    &  &  86.9 & 92.3 & --    & --      \\
				AS-GCN \cite{li2019actional}            &CVPR    & - &  86.8 & 94.2 & 77.9  & 78.5    \\
				2s-AGCN \cite{shi2019two}               &CVPR   & 6.94 &  88.5 & 95.1 & 82.9  & 84.9    \\
				% MS-AAGCN \cite{ms-aagcn}                &TIP     & 14.0 &   90.0 & 96.2 & --    & --      \\
				DGNN \cite{shi2019skeleton}             &CVPR    & 26.24 &  89.9 & 96.1 & --    & --      \\
				% GR-GCN \cite{gao2019optimized}          &ACMMM   &  & 87.5 & 94.3 & --    & --      \\
				% SGN \cite{zhang2020semantics}           &CVPR    &  -- &  89.0 & 94.5	& --    & --\\
				NAS-GCN \cite{peng2020learning}         &AAAI  & 6.57 &  89.4 & 95.7 & --    & --      \\
				2s-Shift-GCN \cite{cheng2020skeleton}   &CVPR    & 1.40 &  89.7 & 96.0 & 85.3  & 86.6    \\
                % ResGCN \cite{ResGCN}                    &ACMMM &  3.64 & 90.9 & 96.0 & 87.3  & 88.3    \\
				MS-G3D \cite{msg3d}                     &CVPR    & 6.40 &  \textbf{91.5} & 96.2 & \textbf{86.9}  & \textbf{88.2}    \\      
				 \midrule
				
				\textbf{LSTA-Net(ours)}          & --   & \textbf{2.10} & 91.2 & \textbf{96.3} & \textbf{86.9} & 87.9  \\
				% \textbf{LSTA-Net (Four Streams)} & ours & \textbf{-}           & \textbf{}   \\
				\bottomrule       
		\end{tabular}}
		\caption{Comparison of the Top-1 accuracy (\%) with the state-of-the-art methods on the NTU RGB+D 60 \& 120 datasets. The top part consists of several models without GCN technique, while the middle part contains some GCN-based models. The recent popular GCN-based models are presented with parameter number (million).}
		\vspace{-0.2cm}
		\label{ntu60,120}
	\end{table*}
	
	
	\begin{table*}[ht!]
		\centering
		\scalebox{0.9}{
			\begin{tabular}{lc|c|cc|cc}
				\toprule
				\multirow{2}{*}{Methods} & \multirow{2}{*}{Publiser} & 
				% \multirow{2}{*}{FLOPs} 
				 \multirow{2}{*}{Param.} & \multicolumn{2}{c}{NTU RGB+D 60} & \multicolumn{2}{c}{NTU RGB+D 120} 
				\\ \cline{4-5} \cline{6-7}  & & & X-Sub & X-View & X-Sub & X-Set    
				\\  \midrule\midrule
				% \multicolumn{8}{c}{CNN and RNN based methods} \\
				% \\ \hline 
				% CNN and RNN based \\ 
				%  HBRNN \cite{du2015hierarchical}         &CVPR    &  &  59.1 & 64.0 & --    & --      \\
			
	
		
				2s-Shift-GCN \cite{cheng2020skeleton}   &CVPR    & 1.40 &  89.7 & 96.0 & 85.3  & 86.6    \\
				4s-Shift-GCN \cite{cheng2020skeleton}   &CVPR    & 2.80 &  90.7 & \textbf{96.5} & 85.9  & 87.6    \\
				 \midrule
				\textbf{LSTA-Net(ours)}          & --   & \textbf{2.10} & \textbf{91.2} & 96.3 & \textbf{86.9} & \textbf{87.9}  \\
				% \textbf{LSTA-Net (Four Streams)} & ours & \textbf{-}           & \textbf{}   \\
				\bottomrule       
		\end{tabular}}

		\vspace{-0.2cm}

	\end{table*}
	
	\subsection{Model Architecture} \label{model_architecture}
	Our LSTA model consists of three modules, including Spatial Decentralized Aggregation (MSA), Temporal Pyramid Aggregation (TPA) and Maximum-response Attention Module (MAM). An overall architecture is demonstrated in Figure\ref{fig:framework}. The SDA module is responsible for exploring the semantically related intrinsic connectivity of the disentangled joints in the spatial domain. The TPA module is capable of modelling the long-range temporal relationships over distant frames. MAM is an efficient attention module, which contains only a handful of parameters, and simultaneously generates new features independent of the known receptive fields of the convolution kernels. The attention module is then attached to the SDA and TPA modules (denote as A-SDA and A-TPA in Fig.(\ref{fig:framework}) to capture local cross-spatial/temporal information interactions respectively. Then, we stack multiple A-SDA and A-TPA units to form a complete network, followed by the global average pooling layer and the fully-connected layer to acquire the classification score $\hat{y}$ of the action. Formally, we have:
	\begin{equation}\label{eq11}
	\hat{y}=f_{\rm{LSTA}}\left(\widetilde{\textbf{A}^{*}};\textbf{X}_{\rm{att}(1)}^{\rm{spat}},\textbf{X}_{\rm{att}(1)}^{\rm{temp}},\dots,\textbf{X}_{\rm{att}(L)}^{\rm{spat}},\textbf{X}_{\rm{att}(L)}^{\rm{temp}}\right),
	\end{equation}
	where $\textbf{X}_{\rm{att}(l)}^{\rm{spat}}$ and $\textbf{X}_{\rm{att}(l)}^{\rm{temp}}$ denote the aggregated spatial and temporal features with the maximum attention modules, respectively. $ \widetilde{\textbf{A}^{*}}=\sum_{k=0}^{K}\widetilde{\textbf{A}_{(k)}^{*}} $, where $ \widetilde{\textbf{A}_{(k)}^{*}} $ represents the sum of the graph Laplacian matrix $ \widehat{\textbf{A}_{(k)}} $ and its mask $ \widehat{\textbf{A}_{(k)}^{\rm{res}}} $. Specifically, $ \widehat{\textbf{A}_{(k)}^{\rm{res}}} $ is a learnable, unconstrained graph residual mask that has been employed in \cite{shi2019skeleton,shi2019two,msg3d} to strengthen, weaken, add, or remove edges dynamically. Mathematically, the normalisation of masked Laplacian graph can be written as:
	\begin{equation}\label{eq12}
	\widetilde{\textbf{A}_{(k)}^{*}}=\widehat{\textbf{D}}_{(k)}^{-\frac{1}{2}}\left(\widehat{\textbf{A}_{(k)}}+\widehat{\textbf{A}_{(k)}^{\rm{res}}}\right)\widehat{\textbf{D}}_{(k)}^{-\frac{1}{2}},
	\end{equation} 
	where the initial value of $ \widehat{\textbf{A}_{(k)}^{\rm{res}}} $ is a minimum value close to zero, and it is expected to slightly correct the edges of the graph by introducing all possible actions for each scale \textit{k}. When there are major defects in the graphic structure, the minor edge correction may be insufficient, but it tends to provide the most appropriate mask for each scale based on the spatial context of the input graph.
	
	In addition, the second-order information (i.e., the lengths and directions of bones) of the original skeleton data is naturally more discriminative for action recognition and is applied to our LSTA model. Inspired by \cite{shi2019skeleton,shi2019two,si2019attention,peng2020learning,msg3d}, we devise our framework in the two-stream fashion where a separate model with an identical architecture is trained by bone features. The initialisation of the bone features is set to the vector difference of adjacent joints directed away from the center of the human body. In order to construct a complete tree-structured skeleton graph, the zero bone vector is initialised at the body center to obtain \textit{N} bones from \textit{N} joints and then we reuse it for connectivity definition. The final predicted probability of a given skeleton sequence is jointly determined by the Softmax scores generated from both joint and bone models.
	
% 	\subsection{Discussion}
% 	In this subsection, a comprehensive and in-depth analysis will be given to show the superiority of our LSTA model. (1) Compare with the disentangled graph in MS-G3D model \cite{msg3d}, our A-SDA module takes into account the attention on the spatial graph, which allows the capture of long-range correlations of joints and then significantly improves the ability to extract high-level spatial semantics (with the need of conjugate transpose so that attention module can be applied to the node dimension). (2) The multi-scale feature aggregation mechanism was first introduced to image-related tasks by \cite{res2net} while our TPA module studies the aggregation of multiple subsets of temporal features. These subsets are formulated as a tree-structured residual architecture so that a series of sub-convolutions are successively applied to the fragmented features and accordingly enlarge the equivalent receiving field in the temporal dimension. Furthermore, in order to guide different groups to capture varied temporal ranges, we utilise dilated convolutions with different dilation rates to construct a temporal pyramid. Moreover, each sub-convolution can be flexibly attached with a local attention module to further improve the ability of long-range interaction. (3) MAM is proposed to adaptively and efficiently capture the arbitrary range of implicit correlations of input data by exploiting cross-channel interaction locally. Considering that the advantage of dilated convolution is able to expand the size of the receiving field without increasing the number of parameters \cite{dilated_cnn}, we have deployed it in both MAM and TPA modules. Consequently, the complete LSTA model can effectively and adaptively learn the short-and long-range of spatial-temporal dependencies with the introduction of countable network parameters.

==> paperSec/relatedwork.tex <==

\section{Related Work}
 Early works of skeleton-based action recognition focus on extracting hand-crafted features from skeletal sequences\cite{vemulapalli2014human,wang2012mining}. Recent works are mainly based on deep learning and can be categorized into three groups: RNNs based methods, CNNs based methods and GNNs/GCNs based methods.

\noindent\textbf{RNNs based methods} first extract skeletal features at every time-step and then utilize RNNs-based sequential model to capture the temporal dependencies\cite{liu2016spatio,song2017end,zheng2019relational}. However, these methods compress the spatial information at every frame and hence the intra-joint dependencies in temporal domain are hard to capture.

\noindent\textbf{CNNs based methods} first transform the skeletons into a vector by their predefined strategies and concatenate the vectors of each frame into a pseudo-image\cite{ke2017new,kim2017interpretable}, and then performs CNNs based image classification. However, as the skeletal data lies in a non-Euclidean space, conventional CNNs approaches are insufficient to capture dependencies between different semantic parts.  

\noindent\textbf{GNN/GCN based methods} express the skeletal data in a graphical space. Most of those works focus on the design of graph structure and effective message passing strategies\cite{defferrard2016convolutional,kipf2016semi}. Recent works are mainly based on GCNs\cite{st_gcn,shi2019two,decouple_gcn_cheng2020eccv}. Some introduce attention mechanisms\cite{shi2019two,ms-aagcn}, or efficient filters \cite{cheng2020skeleton}. Recent MS-G3D\cite{msg3d} introduces a unified module for spatial and temporal modeling. However, its overall structure has multiple pathways and hence overall model is complex. Our method only has single pathway and the factorised strategy achieves comparable performances and keeps more light weight structure.




% The third group of methods that have recently emerged involve the use of GNNs to improve the expressive power of convolution. Specifically, GNN-based approaches can be roughly categorised into two groups: spectral GNNs and spatial GNNs. Spectral GNNs convolve the input graphs with a set of filters based on the Graph Fourier Transform \cite{defferrard2016convolutional,li2018adaptive}. Research in this area predominantly adopted methods such as Chebyshev polynomial approximation \cite{hammond2011wavelets} to alleviate the effect of the computational expense of factoring Laplacian matrices. Spatial GNNs, on the other hand, iteratively learn to aggregate the neighbourhood of each graph node in a layer-wise manner, such as GCN \cite{kipf2016semi} and PSCN \cite{niepert2016learning}. Since then, GCN has been widely adopted to the downstream skeleton-based action recognition tasks. A prominent example is ST-GCN \cite{st_gcn} based on fixed physical graphs. The latest approaches \cite{shi2019skeleton,peng2020learning,shi2019two,tang2018deep} tend to learn an adaptive graph or adopt multi-scale aggregation strategies \cite{li2019actional,li2018spatio,msg3d} for robust feature extraction.  








% 		\subsection{Skeleton-based Action Recognition}
% 			For skeleton-based action recognition, early works focused on extracting hand-crafted features of inputs \cite{vemulapalli2014human,wang2012mining,hussein2013human,du2015hierarchical,song2017end,xie2018memory}. With the help of cost-effective RGB-D sensors, the rapid development of methods based on deep neural networks has revolutionised and reshaped human skeleton-based action recognition. These methods can be broadly categorised into three groups.
	
% 			The first group involves explicitly capturing the sequence properties of actions and modelling their time dependences using RNN or LSTM \cite{du2015hierarchical,ntu_60,liu2016spatio,song2017end,zheng2019relational}. Attempts based on RNN model include constructing an adaptive tree-structured RNN architecture \cite{li2017adaptive} or designing a view adaptation scheme to automatically regulate observation viewpoints during the occurrence of an action \cite{zhang2017view}. As an alternative way to capturing sequential information, LSTM networks have been employed to mine global informative joints \cite{liu2017global}; to extract co-occurrence features of skeleton sequences \cite{zhu2016co} or to learn stacked temporal dynamics \cite{si2018skeleton}. 
	
% 			The second group exploits various predefined transformation rules to treat the input skeleton as a pseudo-image, which is then extracted and purified by a CNN \cite{ke2017new,kim2017interpretable}. Standard works include skepxels \cite{liu2019skepxels}, jointwise co-occurence feature learning \cite{li2018co}, and enhanced skeleton visualization model \cite{liu2017enhanced}. However, conventional CNNs are usually insufficient to accurately express the vertex information located in non-Euclidean space. 
		
% 			The third group of methods that have recently emerged involve the use of GNNs to improve the expressive power of convolution. Specifically, GNN-based approaches can be roughly categorised into two groups: spectral GNNs and spatial GNNs. Spectral GNNs convolve the input graphs with a set of filters based on the Graph Fourier Transform \cite{defferrard2016convolutional,li2018adaptive}. Research in this area predominantly adopted methods such as Chebyshev polynomial approximation \cite{hammond2011wavelets} to alleviate the effect of the computational expense of factoring Laplacian matrices. Spatial GNNs, on the other hand, iteratively learn to aggregate the neighbourhood of each graph node in a layer-wise manner, such as GCN \cite{kipf2016semi} and PSCN \cite{niepert2016learning}. Since then, GCN has been widely adopted to the downstream skeleton-based action recognition tasks. A prominent example is ST-GCN \cite{st_gcn} based on fixed physical graphs. The latest approaches \cite{shi2019skeleton,peng2020learning,shi2019two,tang2018deep} tended to adaptively learn the graph topology or aggregate multi-scale features \cite{li2019actional,msg3d,li2018spatio}.  
		
% 		\subsection{Attention-based Approaches}
% 			Attention mechanisms, which select relatively critical information from all inputs, have been recently presented to improve the performance of categorising skeleton sequences. Early works applied attention mechanisms at multiple levels of the network to distinguish actions based on joints dependencies \cite{song2017end}. Then, \cite{xie2018memory} proposed a temporal-then-spatial recalibration scheme and further boosted it through the memory attention network. Similarly, \cite{liu2017global} aimed to discover informative joints in each frame of each skeleton sequence by using a global context memory cell. Then, Spatial-Temporal Graph Routing (STGR) network \cite{li2019spatio} added additional edges to skeleton graphs with frame-wise attention and global self-attention mechanisms. Analogously, Two-stream adaptive graph convolutional networks (2s-AGCN) \cite{shi2019two} introduced adaptation graphs with self-attention and free-learning graphs as residual masks. Besides, \cite{si2019attention} employed attention-based graph convolutional LSTM to capture co-occurrence relationships in Spatio-temporal domain. More recently, \cite{cho2020self} investigated the effectiveness of modelling spatial-temporal dependencies and capturing long-range correlations by applying self-attention mechanism to the skeleton sequences.   

	
